PARTNR: Pick and place Ambiguity Resolving by Trustworthy iNteractive leaRning

Several recent works show impressive results in mapping language-based human commands and image scene observations to direct robot executable policies (e.g., pick and place poses). However, these approaches do not consider the uncertainty of the trained policy and simply always execute actions suggested by the current policy as the most probable ones. This makes them vulnerable to domain shift and inefficient in the number of required demonstrations. We extend previous works and present the PARTNR algorithm that can detect ambiguities in the trained policy by analyzing multiple modalities in the pick and place poses using topological analysis. PARTNR employs an adaptive, sensitivity-based, gating function that decides if additional user demonstrations are required. User demonstrations are aggregated to the dataset and used for subsequent training. In this way, the policy can adapt promptly to domain shift and it can minimize the number of required demonstrations for a well-trained policy. The adaptive threshold enables to achieve the user-acceptable level of ambiguity to execute the policy autonomously and in turn, increase the trustworthiness of our system. We demonstrate the performance of PARTNR in a table-top pick and place task.

==> results.tex <==
\begin{table}[!t]
  \vspace{-1cm}
  \setlength\tabcolsep{2.3pt}
  \centering
  \hspace*{-1.9cm}
  \scriptsize
\begin{tabular}{lcccccccc}
\toprule
                                                   & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}put-blocks-in-bowls\\seen-colors\end{tabular}}   & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}put-blocks-in-bowls\\\unseen{unseen}-colors\end{tabular}}    \\

  \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21} \cmidrule(lr){22-25}   \\[-5pt]
                       & \multicolumn{1}{c}{1}                & 10                & 100              & 1000              & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{10} & \multicolumn{1}{c}{100} & \multicolumn{1}{c}{1000} \\ \midrule
\transportermodel~\citep{zengTransporterNetworksRearranging2021}                           & 11.7                 & 17.2                 & 14.8                 & 18.7    & 11.7                 & 17.2                 & 14.8                 & 18.7                         \\
\rowcolor[rgb]{0.792,1,0.792} \multicliport & \textbf{32.0}        & \textbf{48.8}        & \textbf{55.3}        & \textbf{45.8}   & \textbf{32.0}        & \textbf{48.8}        & \textbf{55.3}        & \textbf{45.8}                \\
 \bottomrule
\end{tabular}
  \vspace{0.5em}
  \caption{\scriptsize\textbf{Language-Conditioned Test Results.} Task success scores (mean \%) from 100 evaluation instances vs. \# of training demonstrations (1, 10, 100, or 1000). 
  The challenges pertaining to each task are described in \appsecref{app:task_details}.
  \cliportmodel~models are trained on seen splits, and evaluated on both seen and unseen splits.
  \multicliport~models are trained on seen splits of all 10 tasks with $1\mathbb{T}$, $10\mathbb{T}$, $100\mathbb{T}$, and $1000\mathbb{T}$ demonstrations where $\mathbb{T}=10$.
  \multiloo~indicate \multicliport~models trained on seen-and-\unseen{unseen} splits from all tasks \textit{except} for that one particular heldout task, for which it is trained only the seen split.
    See \figref{fig:average_plot} for an overview with average scores.
  }
  \vspace{-4.1em}
\label{table:lang-cond}
\end{table}

==> results_table.tex <==
\begin{table}[!t]
  \vspace{-1cm}
  \setlength\tabcolsep{2.3pt}
  \centering
  \hspace*{-1.9cm}
  \scriptsize
\begin{tabular}{lcccc}
\toprule
                                                   & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}packing-box-pairs\\\seen{seen}-colors\end{tabular}}          & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}packing-box-pairs\\\unseen{unseen}-colors\end{tabular}}     & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}packing-\seen{seen}-google\\objects-seq\end{tabular}} & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}packing-\unseen{unseen}-google\\objects-seq\end{tabular}} & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}packing-\seen{seen}-google\\objects-group\end{tabular}} & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}packing-\unseen{unseen}-google\\objects-group\end{tabular}}  \\
  \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21} \cmidrule(lr){22-25}  \\[-5pt]
Method                 & 1                                   & 10                & 100                & 1000               & \multicolumn{1}{c}{1}                & 10                & 100                & 1000                & \multicolumn{1}{c}{1}               & 10               & 100              & 1000              & \multicolumn{1}{c}{1}               & 10               & 100               & 1000               & \multicolumn{1}{c}{1}                & 10                & 100              & 1000              & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{10} & \multicolumn{1}{c}{100} & \multicolumn{1}{c}{1000} \\ \midrule
\transportermodel~\citep{zengTransporterNetworksRearranging2021}                             & 44.2                 & 55.2                 & 54.2                 & 52.4                        & 34.6                 & 48.7                 & 47.2                 & 54.1                          & 26.2                 & 39.7                 & 45.4                 & 46.3                    & 19.9                 & 29.8                 & 28.7                 & 37.3                      & 60.0                 & 54.3                 & 61.5                 & 59.9                      & 46.2                 & 54.7                 & 49.8                 & 52.0                         \\
\clipmodel                                    & 38.6                 & 69.7                 & 88.5                 & 87.1                        & 33.0                 & 65.5                 & 68.8                 & 61.2                          & 29.1                 & 67.9                 & \textbf{89.3}        & 95.8                    & 37.1                 & 49.4                 & 60.4                 & 57.8                      & 52.5                 & 62.0                 & \textbf{89.6}        & \textbf{92.7}             & 43.4                 & 65.9                 & 73.1                 & 70.0                         \\
\rnbertmodel~                                     & 36.2                 & 64.0                 & \textbf{94.7}        & 90.3                        & 31.4                 & 52.7                 & 65.6                 & \textbf{72.1}                 & 32.9                 & 48.4                 & 87.9                 & 94.0                    & 29.3                 & 48.5                 & 48.3                 & 56.1                      & 46.4                 & 52.9                 & 76.5                 & 86.4                      & 43.2                 & 52.0                 & 66.3                 & 73.7                         \\
\cliportmodel~                                     & 51.6                 & 82.9                 & 92.7                 & \textbf{98.2}               & 45.6                 & 65.3                 & 68.6                 & 71.5                          & 14.8                 & 59.5                 & 86.8                 & \textbf{96.2}           & 27.2                 & 50.0                 & 65.5                 & \textbf{71.9}             & 52.7                 & 67.0                 & 84.1                 & 94.0                      & 61.5                 & 66.2                 & 78.4                 & \textbf{81.5}                \\
\rowcolor[rgb]{0.792,1,0.792} \multicliport~ & \textbf{66.8}        & \textbf{88.6}        & 94.1                 & 96.6                        & \textbf{59.0}        & \textbf{69.7}        & \textbf{76.2}        & 71.4                          & \textbf{41.6}        & \textbf{78.4}        & 85.0                 & 84.4                    & \textbf{40.7}        & \textbf{51.1}        & \textbf{65.8}        & 70.3                      & \textbf{71.3}        & \textbf{84.6}        & \textbf{89.6}        & 88.3                      & \textbf{68.4}        & \textbf{69.6}        & \textbf{78.4}        & 80.3                         \\
\rowcolor[rgb]{0.933,0.933,1} \multiloo~     & –                    & –                    & –                    & –                           & \textit{46.2}        & \textit{72.0}        & \textit{86.2}        & \textit{80.3}                 & –                    & –                    & –                    & –                       & \textit{35.4}        & \textit{45.1}        & \textit{78.9}        & \textit{87.4}             & –                    & –                    & –                    & –                         & \textit{48.6}        & \textit{69.3}        & \textit{84.8}        & \textit{89.1}                \\ 
      \midrule
                                                   & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}stack-block-pyramid\\seq-\seen{seen}-colors\end{tabular}}      & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}stack-block-pyramid\\seq-\unseen{unseen}-colors\end{tabular}} & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}separating-piles\\\seen{seen}-colors\end{tabular}}    & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}separating-piles\\\unseen{unseen}-colors\end{tabular}}    & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}towers-of-hanoi\\seq-\seen{seen}-colors\end{tabular}}   & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}towers-of-hanoi\\seq-\unseen{unseen}-colors\end{tabular}}    \\

  \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21} \cmidrule(lr){22-25} \\[-5pt]
                       & 1                                   & 10                & 100                & 1000               & \multicolumn{1}{c}{1}                & 10                & 100                & 1000                & \multicolumn{1}{c}{1}               & 10               & 100              & 1000              & \multicolumn{1}{c}{1}               & 10               & 100               & 1000               & \multicolumn{1}{c}{1}                & 10                & 100              & 1000              & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{10} & \multicolumn{1}{c}{100} & \multicolumn{1}{c}{1000} \\ \midrule
\transportermodel~\citep{zengTransporterNetworksRearranging2021}                             & 4.5                  & 2.3                  & 5.2                  & 4.5                         & 3.0                  & 4.0                  & 2.3                  & 5.8                           & 42.7                 & 52.3                 & 42.0                 & 48.4                    & 41.2                 & 49.2                 & 44.7                 & 52.3                      & 25.4                 & 67.9                 & 98.0                 & 99.9                      & 24.3                 & 44.6                 & 71.7                 & 80.7                         \\
\clipmodel                                    & 6.3                  & 28.7                 & 55.7                 & 54.8                        & 2.0                  & 12.2                 & 18.3                 & 19.5                          & 43.5                 & 55.0                 & 84.9                 & 90.2                    & \textbf{59.9}        & 49.6                 & 73.0                 & 71.0                      & 9.4                  & 52.6                 & 88.6                 & 45.3                      & 24.7                 & 47.0                 & 67.0                 & 58.0                         \\
\rnbertmodel~                                     & 5.3                  & 35.0                 & 89.0                 & 97.5                        & 6.2                  & 12.2                 & 21.5                 & 30.7                          & 31.8                 & 47.8                 & 46.5                 & 46.5                    & 33.4                 & 44.4                 & 41.3                 & 44.9                      & 28.0                 & 66.1                 & 91.3                 & 92.1                      & 17.4                 & 75.1                 & 85.3                 & 89.3                         \\
\cliportmodel~                                     & 28.3                 & 64.7                 & 93.3                 & \textbf{98.8}               & 13.7                 & 24.3                 & 31.2                 & \textbf{41.3}                 & \textbf{54.5}        & 59.5                 & \textbf{93.1}        & \textbf{98.0}           & 47.2                 & 51.0                 & \textbf{76.6}        & \textbf{75.2}             & 59.4                 & 92.9                 & 97.4                 & \textbf{100}              & 56.1                 & \textbf{89.7}        & \textbf{95.9}        & \textbf{99.4}                \\
\rowcolor[rgb]{0.792,1,0.792} \multicliport~ & \textbf{33.5}        & \textbf{75.3}        & \textbf{96.8}        & 96.5                        & \textbf{23.3}        & \textbf{26.8}        & \textbf{31.7}        & 22.2                          & 48.9                 & \textbf{72.4}        & 90.3                 & 89.0                    & 56.6                 & \textbf{62.6}        & 64.9                 & 62.8                      & \textbf{61.6}        & \textbf{96.3}        & \textbf{98.7}        & 98.1                      & \textbf{60.1}        & 65.6                 & 76.7                 & 68.7                         \\
\rowcolor[rgb]{0.933,0.933,1} \multiloo~     & –                    & –                    & –                    & –                           & \textit{15.5}        & \textit{51.5}        & \textit{59.3}        & \textit{79.8}                 & –                    & –                    & –                    & –                       & \textit{49.9}        & \textit{51.8}        & \textit{48.2}        & \textit{59.8}             & –                    & –                    & –                    & –                         & \textit{56.7}        & \textit{78.0}        & \textit{88.3}        & \textit{96.9}                \\  
         \midrule
                                                   & \multicolumn{4}{c}{align-rope}                                                                        & \multicolumn{4}{c}{packing-\unseen{unseen}-shapes}                                                          & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}assembling-kits-seq\\\seen{seen}-colors\end{tabular}} & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}assembling-kits-seq\\\unseen{unseen}-colors\end{tabular}} & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}put-blocks-in-bowls\\\seen{seen}-colors\end{tabular}}   & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}put-blocks-in-bowls\\\unseen{unseen}-colors\end{tabular}}    \\

  \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21} \cmidrule(lr){22-25}   \\[-5pt]
                       & 1                                   & 10                & 100                & 1000               & \multicolumn{1}{c}{1}                & 10                & 100                & 1000                & \multicolumn{1}{c}{1}               & 10               & 100              & 1000              & \multicolumn{1}{c}{1}               & 10               & 100               & 1000               & \multicolumn{1}{c}{1}                & 10                & 100              & 1000              & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{10} & \multicolumn{1}{c}{100} & \multicolumn{1}{c}{1000} \\ \midrule
\transportermodel~\citep{zengTransporterNetworksRearranging2021}                             & 6.9                  & 30.6                 & 33.1                 & 51.5                        & 16.0                 & 20.0                 & 22.0                 & 22.0                          & 5.8                  & 11.6                 & 28.6                 & 29.6                    & 7.8                  & 17.6                 & 25.6                 & 28.4                      & 16.8                 & 33.3                 & 62.7                 & 64.7                      & 11.7                 & 17.2                 & 14.8                 & 18.7                         \\
\clipmodel                                    & 13.4                 & 48.7                 & 70.4                 & 70.7                        & 13.0                 & 28.0                 & \textbf{44.0}        & \textbf{50.0}                 & 0.8                  & 9.2                  & 19.8                 & 23.0                    & 2.0                  & 4.6                  & 10.8                 & 19.8                      & 23.5                 & 60.2                 & 93.5                 & 97.7                      & 11.2                 & 34.2                 & 33.2                 & 44.5                         \\
\rnbertmodel~                                     & 3.1                  & 25.0                 & 63.8                 & 57.1                        & 19.0                 & 25.0                 & 32.0                 & 44.0                          & 2.2                  & 5.6                  & 11.6                 & 21.8                    & 1.6                  & 6.4                  & 10.4                 & 18.4                      & 13.8                 & 44.5                 & 81.2                 & 91.8                      & 16.2                 & 23.0                 & 30.3                 & 23.8                         \\
\cliportmodel                                     & \textbf{20.1}        & \textbf{77.4}        & \textbf{85.6}        & \textbf{95.4}               & 21.0                 & 26.0                 & 40.0                 & 37.0                          & \textbf{12.2}        & 17.8                 & \textbf{47.0}        & \textbf{66.6}           & \textbf{16.2}        & 18.0                 & \textbf{35.4}        & \textbf{34.8}             & 23.5                 & 68.3                 & 92.5                 & \textbf{100}              & 18.0                 & 35.3                 & 37.3                 & 25.0                         \\
\rowcolor[rgb]{0.792,1,0.792} \multicliport & 19.6                 & 49.3                 & 82.4                 & 74.9                        & \textbf{25.0}        & \textbf{35.0}        & 37.0                 & 31.0                          & 11.4                 & \textbf{34.8}        & 46.2                 & 52.4                    & 7.8                  & \textbf{21.6}        & 29.0                 & 25.4                      & \textbf{54.0}        & \textbf{90.2}        & \textbf{99.5}        & \textbf{100}              & \textbf{32.0}        & \textbf{48.8}        & \textbf{55.3}        & \textbf{45.8}                \\
\rowcolor[rgb]{0.933,0.933,1} \multiloo     & –                    & –                    & –                    & –                           & –                    & –                    & –                    & –                             & –                    & –                    & –                    & –                       & \textit{7.6}         & \textit{10.4}        & \textit{43.8}        & \textit{34.6}             & –                    & –                    & –                    & –                         & \textit{23.0}        & \textit{41.8}        & \textit{66.5}        & \textit{75.7}                \\
 \bottomrule
\end{tabular}
  \vspace{0.5em}
  \caption{\scriptsize\textbf{Language-Conditioned Test Results.} Task success scores (mean \%) from 100 evaluation instances vs. \# of training demonstrations (1, 10, 100, or 1000). 
  The challenges pertaining to each task are described in \appsecref{app:task_details}.
  \cliportmodel~models are trained on \seen{seen} splits, and evaluated on both \seen{seen} and \unseen{unseen} splits.
  \multicliport~models are trained on \seen{seen} splits of all 10 tasks with $1\mathbb{T}$, $10\mathbb{T}$, $100\mathbb{T}$, and $1000\mathbb{T}$ demonstrations where $\mathbb{T}=10$.
  \multiloo~indicate \multicliport~models trained on \seen{seen}-and-\unseen{unseen} splits from all tasks \textit{except} for that one particular heldout task, for which it is trained only the \seen{seen} split.
    See \figref{fig:average_plot} for an overview with average scores.
  }
  \vspace{-4.1em}
\label{table:lang-cond}
\end{table}
